Encodings of Bounded Synthesis

The reactive synthesis problem is to compute a system satisfying a given specification in temporal logic. Bounded synthesis is the approach to bound the maximum size of the system that we accept as a solution to the reactive synthesis problem. As a result, bounded synthesis is decidable whenever the corresponding verification problem is decidable, and can be applied in settings where classic synthesis fails, such as in the synthesis of distributed systems. In this paper, we study the constraint solving problem behind bounded synthesis. We consider different reductions of the bounded synthesis problem of linear-time temporal logic (LTL) to constraint systems given as boolean formulas (SAT), quantified boolean formulas (QBF), and dependency quantified boolean formulas (DQBF). The reductions represent different trade-offs between conciseness and algorithmic efficiency. In the SAT encoding, both inputs and states of the system are represented explicitly; in QBF, inputs are symbolic and states are explicit; in DQBF, both inputs and states are symbolic. We evaluate the encodings systematically using benchmarks from the reactive synthesis competition (SYNTCOMP) and state-of-the-art solvers. Our key, and perhaps surprising, empirical finding is that QBF clearly dominates both SAT and DQBF.

==> tikz/product-arbiter.tex <==
\tikzset{
state/.style={rounded corners,rectangle split, rectangle split parts=2, inner sep=3pt, draw}
}
\scalebox{.87}{
\begin{tikzpicture}[node distance=2cm and 2.5cm,auto,thick]
	\node[state] (00) {$\langle t_0, q_0 \rangle \mid g_1$ \nodepart{two} $\lambda^{\#}: 0 $};
	
	\node[state, below=of 00] (1012) {$\langle t_1, q_0, q_1, q_2 \rangle \mid g_2$ \nodepart{two} $\lambda^{\#}: (0,2,1) $};
	\node[state, left=of 1012] (101) {$\langle t_1, q_0, q_1 \rangle \mid g_2$ \nodepart{two} $\lambda^{\#}: (0,2) $};
	\node[state, right=of 1012] (102) {$\langle t_1, q_0, q_2 \rangle  \mid g_2$ \nodepart{two} $\lambda^{\#}: (0,1) $};
	\path[->] (00) edge node[right] {$r_1 r_2$} (1012);
	\path[->] (00) edge [bend right=10] node[left,outer sep=3pt] {$r_1 \overline{r_2}$} (101);
	\path[->] (00) edge [bend left=10] node[right,outer sep=3pt] {$\overline{r_1} r_2$} (102);
	
	\node[state, below=of 1012] (0012) {$\langle t_0, q_0, q_1, q_2 \rangle  \mid g_1$ \nodepart{two} $\lambda^{\#}: (0,1,2) $};
	\path[<->] (1012) edge node[right,near end] {$r_1 r_2$} (0012);
	\path[->] (101) edge[bend right=10] node[below,very near end] {$r_2$} (0012);
	\path[->] (102) edge[bend left=10] node[right,very near end,outer sep=3pt] {$r_1 r_2$} (0012);
	
	\node[state, left=of 0012] (001) {$\langle t_0, q_0, q_1 \rangle \mid g_1$ \nodepart{two} $\lambda^{\#}: (0,1) $};	
	\node[state, right=of 0012] (002) {$\langle t_0, q_0, q_2 \rangle \mid g_1$ \nodepart{two} $\lambda^{\#}: (0,2) $};
	\path[<->] (101) edge node[left] {$r_1 \overline{r_2}$} (001);
	\path[<->] (102) edge node[right] {$\overline{r_1} r_2$} (002);
	\path[->] (001) edge node[left,very near end, outer sep=3pt] {$r_1 r_2$} (1012);
	\path[->] (002) edge node[left,very near end, outer sep=4pt] {$r_1 r_2$} (1012);
	
	\node[state, below=of 0012] (10) {$\langle t_1, q_0 \rangle \rangle \mid g_2$ \nodepart{two} $\lambda^{\#}: 0 $};
	\path[<->,draw] (00) .. controls ($(00.east)+(8,0)$)  and ($(10.east)+(8,0)$) ..  node[right] {$\overline{r_1 r_2}$} (10);
	
	\path[->] (1012) edge[bend right=25] node[right,very near end,outer sep=3pt] {$\overline{r_2}$} (001);
	\path[->] (1012) edge[bend left=25] node[left,very near end] {$\overline{r_1}r_2$} (002);
	\path[->] (002) edge[bend left=15] node[right,near end,outer sep=3pt] {$\overline{r_1 r_2}$} (10);
	\path[->] (001) edge[bend right=15] node[left,near end,outer sep=3pt] {$\overline{r_1 r_2}$} (10);
	
	\path[->] (0012) edge node[above,very near end] {$\overline{r_1}$} (102);
	
	\path[->] (102) edge node[below,very near end,outer sep=3pt] {$r_1\overline{r_2}$} (001);
	\path[->] (001) edge [bend left=5] node[above,very near end,outer sep=3pt] {$\overline{r_1}r_2$} (102);
	
	\path[->] (10) edge[bend right=15] node[right,near end,outer sep=3pt] {$r_1\overline{r_2}$} (001);
	\path[->] (10) edge node[right] {$r_1 r_2$} (0012);
	\path[->] (10) edge[bend left=15] node[left,near end,outer sep=3pt] {$\overline{r_1} r_2$} (002);
	
	\draw (00) edge[<-] +(-1.5,0.75);
\end{tikzpicture}
}
